SparseFusion: Distilling View-conditioned Diffusion for 3D Reconstruction

We propose SparseFusion, a sparse view 3D reconstruction approach that unifies recent advances in neural rendering and probabilistic image generation. Existing approaches typically build on neural rendering with re-projected features but fail to generate unseen regions or handle uncertainty under large viewpoint changes. Alternate methods treat this as a (probabilistic) 2D synthesis task, and while they can generate plausible 2D images, they do not infer a consistent underlying 3D. However, we find that this trade-off between 3D consistency and probabilistic image generation does not need to exist. In fact, we show that geometric consistency and generative inference can be complementary in a mode-seeking behavior. By distilling a 3D consistent scene representation from a view-conditioned latent diffusion model, we are able to recover a plausible 3D representation whose renderings are both accurate and realistic. We evaluate our approach across 51 categories in the CO3D dataset and show that it outperforms existing methods, in both distortion and perception metrics, for sparse-view novel view synthesis.

==> modules/figure-ablation1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% ABLATION 1 %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering 
\vspace{-0.5mm}
\includegraphics[width=1.0\linewidth]{figures/test_plot_ab_r1.jpg}
\vspace{-8mm}
\captionof{figure}{
    \textbf{Ablation on Distillation Methods} We show metrics for scenes optimized with different distillation losses and setups. 
} 
\label{fig:ablation1}
\vspace{0mm}
\end{figure}

==> modules/figure-ablation2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% ABLATION 2 %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering 
\vspace{-0.5mm}
\includegraphics[width=1.0\linewidth]{figures/test_plot_ab2.jpg}
\captionof{figure}{
    \textbf{The Importance of Probabilistic Mode Seeking.} We show metrics on optimized 3D scene with three setups: C-GPNR, V-LDM, and V-LDM distillation. \TODO{NEED TO UPDATE PLOT}
} 
\label{fig:ablation1}
\vspace{3mm}
\end{figure}

==> modules/figure-fail.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/fail.pdf}
    % \vspace{-2mm}
    \caption{
    \textbf{Failure Modes.} Top: since VLDM and Instant NGP is trained with black background color, sometimes we fail to disambiguate a black foreground object and a black background. Bottom: the category for remote is biased towards TV remotes and our model propagates that bias in synthesized views. }
    \vspace \figmargin
    \label{fig:mode}
    % \figlabel{overview_p1}
\end{figure} 

==> modules/table-co3d-10-backup.tex <==
%------------------------------------------------------------------------
\begin{table}[t!]
\footnotesize
\begin{center}
\caption{\textbf{View Synthesis on 10 Categories.} We benchmark view synthesis results on the 10 categories with 2, 3, and 6 input views.  }
\label{tab:co3d-10}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l cc cc cc}
\toprule
& \multicolumn{2}{c}{2 Views} & \multicolumn{2}{c}{3 Views} & \multicolumn{2}{c}{6 Views}\\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
& PSNR $\shortuparrow$ & LPIPS $\shortdownarrow$  & PSNR $\shortuparrow$ & LPIPS $\shortdownarrow$ & PSNR $\shortuparrow$ & LPIPS $\shortdownarrow$ \\
\midrule
PixelNeRF \cite{yu2021pixelnerf}       

& 19.52 & 0.327 & 20.67 & 0.293 & 22.47 & 0.241  \\

NerFormer \cite{reizenstein2021common}       

% CORRECTION FOR TYPO 12-4-2022
% ORIGINAL
% & 17.88 & 0.382 & 18.54 & 0.367 & 19.72 & 0.266 \\
% CORRECTED
& 17.88 & 0.382 & 18.54 & 0.367 & 19.99 &  0.332 \\

ViewFormer\textsuperscript{\ref{fn:one}} \cite{kulhanek2022viewformer}      

& 18.37 & 0.282 & 18.91 & 0.275 & 19.72 & 0.266  \\

EFT                   

& \second 20.85 & 0.289 & \first \textbf{22.71} & 0.262 & \first \textbf{24.57} & 0.210  \\

VLDM                     

& 19.55 & \second 0.247 & 20.85 & \second 0.225 & 22.35 & \second 0.201  \\

SparseFusion            

& \first \textbf{21.34} & \first \textbf{0.225} & \second 22.35 & \first \textbf{0.216} & \second 23.74 & \first \textbf{0.200}  \\

\bottomrule
\vspace{-3em}
\end{tabular}
}
\end{center}
\end{table}

%------------------------------------------------------------------------

==> modules/table-co3d-10.tex <==
%------------------------------------------------------------------------
\begin{table}[t!]
\footnotesize
\begin{center}
\caption{\textbf{View Synthesis on 10 Categories.} We benchmark view synthesis results on the 10 categories with 2, 3, and 6 input views.  }
\label{tab:co3d-10}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l ccc ccc ccc}
\toprule
& \multicolumn{3}{c}{2 Views} & \multicolumn{3}{c}{3 Views} & \multicolumn{3}{c}{6 Views}\\
\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
& PSNR $\shortuparrow$ & SSIM $\shortuparrow$ & LPIPS $\shortdownarrow$  & PSNR $\shortuparrow$ & SSIM $\shortuparrow$ & LPIPS $\shortdownarrow$ & PSNR $\shortuparrow$ & SSIM $\shortuparrow$ & LPIPS $\shortdownarrow$ \\
\midrule
PixelNeRF \cite{yu2021pixelnerf}       

& 19.52 & 0.667 & 0.327 & 20.67 & 0.712 & 0.293 & 22.47 & 0.776 & 0.241  \\

NerFormer \cite{reizenstein2021common}       

% CORRECTION FOR TYPO 12-4-2022
% ORIGINAL
% & 17.88 & 0.382 & 18.54 & 0.367 & 19.72 & 0.266 \\
% CORRECTED
& 17.88 & 0.598 & 0.382 & 18.54 & 0.618 & 0.367 & 19.99 & 0.661 &  0.332 \\

ViewFormer\textsuperscript{\ref{fn:one}} \cite{kulhanek2022viewformer}      

& 18.37 & 0.697 & 0.282 & 18.91 & 0.704 & 0.275 & 19.72 & 0.717 & 0.266  \\

EFT                   

& \second 20.85 & 0.680 & 0.289 & \first \textbf{22.71} & 0.747 & 0.262 & \first \textbf{24.57} & 0.804 & 0.210  \\

VLDM                     

& 19.55 & 0.711 & \second 0.247 & 20.85 & 0.737 & \second 0.225 & 22.35 & 0.768 & \second 0.201  \\

SparseFusion            

& \first \textbf{21.34} & 0.752 & \first \textbf{0.225} & \second 22.35 & 0.766 & \first \textbf{0.216} & \second 23.74 & 0.791 & \first \textbf{0.200}  \\

\bottomrule
\vspace{-3em}
\end{tabular}
}
\end{center}
\end{table}

%------------------------------------------------------------------------

==> modules/table-co3d-50.tex <==
%------------------------------------------------------------------------
\begin{table}
\footnotesize
\begin{center}

\caption{\textbf{View Synthesis on 51 Categories.} We benchmark novel view synthesis on all CO3D categories with 2 input views. }
\label{tab:co3d-50}
\begin{tabular}{l ccc}
\toprule
& \multicolumn{3}{c}{2 Views} \\
\cmidrule(r){2-4}
& PSNR $\shortuparrow$ & SSIM $\shortuparrow$ & LPIPS $\shortdownarrow$ \\
\midrule
NerFormer \cite{reizenstein2021common}           

& 18.44 & 0.614 & 0.365   \\

ViewFormer\textsuperscript{\ref{fn:one}} \cite{kulhanek2022viewformer}         

& 18.91 & 0.718 & 0.265  \\

EFT                         

& \first \textbf{21.44} & 0.719 & 0.281 \\

VLDM                       

& 19.85 & \second 0.732 & \second 0.229   \\

SparseFusion                

& \second 21.20 & \first \textbf{0.756} & \first \textbf{0.223}   \\

\bottomrule
\vspace{-3.5em}
\end{tabular}
\end{center}
\end{table}
%------------------------------------------------------------------------

==> modules/table-srn.tex <==
%------------------------------------------------------------------------
\begin{table}
\footnotesize

\begin{center}

\caption{SRN Cars and Chairs. Category-specific 2-view reconstruction benchmark. We evaluate on the first 20 test scenes for each category with two random input views. \TODO{Cars have a lot of 'white' color which is similar to background, resulting in artifacts. Chairs work fine. Will investigate low PSNR of other methods on chairs.}}
\label{tab:intro}

\begin{tabular}{llcc}
\toprule
& & \multicolumn{2}{c}{2 Views} \\
\cmidrule(r){3-4}
& & PSNR $\shortuparrow$ & LPIPS $\shortdownarrow$ \\
\midrule
\multirow{4}{*}{Cars}
    & PixelNeRF \cite{}     & 24.21 & 0.102 \\
    & EPT        & 23.95 & 0.123 \\
    & VLDM                   & 22.37 & 0.103 \\
    & SparseFusion          & 23.15 & 0.114 \\
\midrule
\multirow{4}{*}{Chairs}
    & PixelNeRF \cite{}     & 20.30 & 0.150 \\
    & EPT       & 21.05 & 0.156 \\
    & VLDM                   & 19.73 & 0.111 \\
    & SparseFusion          & \textbf{21.55} & \textbf{0.102} \\
\bottomrule
\end{tabular}

\end{center}
\end{table}
%------------------------------------------------------------------------

==> rebuttal/figure8_2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% VIEW ANGLE PLOTS %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\centering 
\includegraphics[width=1.0\linewidth]{rebuttal/test_plot_3.jpg}
\vspace{-7mm}
\captionof{figure}{
    Metrics by viewpoint change for additional baselines. 
} 
\figlabel{supp-view-angles}
\vspace{-6.5mm}
\end{figure}

==> rebuttal/rebuttal_metric.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% VIEW ANGLE PLOTS %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\centering 
\vspace{-0.5mm}
\includegraphics[width=1.0\linewidth]{rebuttal/rebuttal_metric_figure.pdf}
\vspace{-7mm}
\captionof{figure}{
    PSNR can reward blurry outputs unlike SSIM, LPIPS. 
} 
\figlabel{supp-metric}
\vspace{-3mm}
\end{figure}

==> rebuttal/ssim.tex <==
%------------------------------------------------------------------------
\begin{table}
\footnotesize

\begin{center}

\definecolor{first}{rgb}{1.0, .83, 0.3}
\definecolor{second}{rgb}{1.0, 0.93, 0.7}
% \definecolor{second}{rgb}{1.0, 0.88, 0.51}
% \definecolor{third}{rgb}{1.0, 0.93, 0.7}
\def \first {\cellcolor{first}}
\def \second {\cellcolor{second}}

\caption{Additional metrics averaged across 10 categories. Note that FID is computed at a set-level (per-category renderings).}

\scriptsize
\vspace{-1em}
\tablelabel{ssim}
\begin{tabular}{l ccc | c}
\toprule
& \multicolumn{4}{c}{2 Views} \\
\cmidrule(r){2-5}
& PSNR $\shortuparrow$ & SSIM $\shortuparrow$ & LPIPS $\shortdownarrow$ & FID $\shortdownarrow$ \\
\midrule
PixelNeRF           

& 19.52 & 0.667 & 0.327 & 250.1   \\

NerFormer           

& 17.88 & 0.598 & 0.382 & 256.7   \\

ViewFormer      

& 18.37 & 0.697 & 0.282 & 163.6  \\

EFT                         

& \second 20.85 & 0.680 & 0.289 & 189.6 \\

VLDM                       

& 19.55 & \second 0.711 & \second 0.247 & \first \textbf{99.6} \\

SparseFusion                

& \first \textbf{21.34} & \first \textbf{0.752} & \first \textbf{0.225} & \second 122.7   \\

\bottomrule
\vspace{-3.5em}
\end{tabular}
\end{center}
\end{table}
%------------------------------------------------------------------------

==> rebuttal/ssim_51cat.tex <==
%------------------------------------------------------------------------
\begin{table}
\footnotesize

\begin{center}

\definecolor{first}{rgb}{1.0, .83, 0.3}
\definecolor{second}{rgb}{1.0, 0.93, 0.7}
% \definecolor{second}{rgb}{1.0, 0.88, 0.51}
% \definecolor{third}{rgb}{1.0, 0.93, 0.7}
\def \first {\cellcolor{first}}
\def \second {\cellcolor{second}}

\caption{We show novel view synthesis metrics on 51 categories and 2 input views. }

\scriptsize
\vspace{-1em}
\tablelabel{ssim}
\begin{tabular}{l ccc}
\toprule
& \multicolumn{3}{c}{2 Views} \\
\cmidrule(r){2-4}
& PSNR $\shortuparrow$ & SSIM $\shortuparrow$ & LPIPS $\shortdownarrow$ \\
\midrule

NerFormer           

& 18.44 & 0.614 & 0.365   \\

ViewFormer      

& 18.91 & 0.718 & 0.265  \\

EFT                         

& \first \textbf{21.44} & 0.719 & 0.281 \\

VLDM                       

& 19.85 & \second 0.732 & \second 0.229  \\

SparseFusion                

& \second 21.20 & \first \textbf{0.756} & \first \textbf{0.223}   \\

\bottomrule
\vspace{-3.5em}
\end{tabular}
\end{center}
\end{table}
%------------------------------------------------------------------------
